Graph Partitioning with Demands: Generalized Conductance and its Applications

We study various graph partitioning tasks subject to general demands. In Graph Partitioning with Demands (GPD), the goal is to delete minimum cost supply edge set so that each remaining component contains at most a prescribed fraction of the total demand. In the hierarchical analogue of this problem, Hierarchical Clustering with Demands (HCD), the goal is to build a hierarchy of clusters, charging each supply edge by the demand in the smallest cluster containing its endpoints. Our main general-graph results are approximation algorithms for GPD and HCD. For every fixed $0<\rho<\eta<1$, we give a polynomial-time bi-criteria algorithm for GPD whose components have demand at most $\eta \cdot W$ and cost at most $\mathcal{O}_{\rho,\eta}(\sqrt{\log n})$ times the optimum cost for threshold~$\rho$. This procedure can then be applied recursively to obtain an $\mathcal{O}(\sqrt{\log n})$-approximation for HCD. The algorithm for GPD itself uses a crucial subproblem called Generalized Conductance (GC), a new generalization of the Sparsest Cut. On supply trees, we show that GC can be solved exactly in polynomial time. We also give bi-criteria algorithms for GPD based on anchored-LP rounding and separator recursion, as well as a single-criterion $(4+\epsilon)$-approximation in $n^{O(1/\rho)}$ time. Moreover, through previous reduction, these GPD algorithms yield a $\frac{4e}{e-1}$-approximation for HCD on trees. We also prove that HCD and GPD and GC are SSEH-hard to approximate within any constant factor. On trees, assuming the Unique Games Conjecture (UGC), GPD is hard to approximate within a factor of $2-\epsilon$ by reduction from Vertex Cover, while HCD is hard to approximate within a factor of $1.0748$, by reduction from Min-Sum Vertex Cover.

==> algorithms/weighted_budget_dp.tex <==
\begin{algorithm}[tbp]
    \caption{Weighted-budget dynamic program on a tree}
    \textbf{Input} Supply tree $T=(V,E,c)$, non-negative integer vertex weights $a(v)\leq L$, and integer budget $L$\;
    \textbf{Output} A minimum-cost edge set $C\subseteq E$ such that every component $H$ satisfies $\sum_{v\in V_H}a(v)\leq L$\;
    Root $T$ at an arbitrary vertex $r$\;
    \ForEach{vertex $v$ in a bottom-up traversal of $T$}{
        Let $u_1,\ldots,u_k$ be the children of $v$\;
        Initialize $F_v^{(0)}(\ell)\gets0$ if $\ell=a(v)$ and $F_v^{(0)}(\ell)\gets+\infty$ otherwise, for $0\leq\ell\leq L$\;
        \For{$j=1,\ldots,k$}{
            \For{$\ell=0,\ldots,L$}{
                Set $\displaystyle F_v^{(j)}(\ell)\gets\min\brc{F_v^{(j-1)}(\ell)+c(vu_j)+F_{u_j},\min_{\substack{0\leq\ell_1,\ell_2\leq L,\ \ell_1+\ell_2=\ell}}\brc{F_v^{(j-1)}(\ell_1)+F_{u_j}(\ell_2)}}$\;
                Store a minimizing choice for state $\ell$\;
            }
        }
        Set $F_v(\ell)\gets F_v^{(k)}(\ell)$ for all $0\leq\ell\leq L$ and $F_v\gets\min_{0\leq b\leq L}\brc{F_v(b)}$\;
    }
    Choose $\ell^*\in\arg\min_{0\leq\ell\leq L}\brc{F_r(\ell)}$ and backtrack from $(r,\ell^*)$ through the stored choices to recover the edge set $C$\;
    \textbf{return} $C$\;
\end{algorithm}


==> algorithms/weighted_budget_recursive.tex <==
\begin{algorithm}[tbp]
    \caption{Recursive weighted-budget partitioning}
    \textbf{Input} Supply tree $T=(V,E,c)$, demand graph $(V,D,w)$, and rational parameters $0<\rho<\eta<1$ and $\alpha\in(1/2,1)$\;
    \textbf{Output} An $\eta$-feasible supply-edge set $C\subseteq E$\;
    \If{$W=0$}{
        \textbf{return} $C=\emptyset$\;
    }
    Set $B_\rho\gets\rho W$ and $B_\eta\gets\eta W$\;
    \textbf{Procedure} $\textsc{WeightedBudgetRecursive}(H)$\;
    \Indp
        \If{$w\br{V_H}\leq B_\eta$}{
            \textbf{return} $\emptyset$\;
        }
        Set $\rho_H\gets B_\rho/w\br{V_H}$ and $\sigma_H\gets\alpha+(1-\alpha)\rho_H$\;
        Run the direct weighted-budget procedure using the local weighted demand degrees on the instance induced by $V_H$ with parameters $\rho_H,\sigma_H$. Let $F_H$ be its returned supply-edge set\;
        Set $C_H\gets F_H$\;
        \ForEach{component $H'$ of $H\setminus F_H$ with $w\br{V_{H'}}>B_\eta$}{
            $C_H\gets C_H\cup\textsc{WeightedBudgetRecursive}(H')$\;
        }
        \textbf{return} $C_H$\;
    \Indm
    $C\gets\textsc{WeightedBudgetRecursive}(T)$\;
    \textbf{return} $C$\;
\end{algorithm}
